On-The-Fly Control of Unknown Systems: From Side Information to Performance Guarantees through Reachability

We develop data-driven algorithms for reachability analysis and control of systems with a priori unknown nonlinear dynamics. The resulting algorithms not only are suitable for settings with real-time requirements but also provide provable performance guarantees. To this end, they merge noisy data from only a single finite-horizon trajectory and, if available, various forms of side information. Such side information may include knowledge of the regularity of the dynamics, algebraic constraints on the states, monotonicity, or decoupling in the dynamics between the states. Specifically, we develop two algorithms, $\texttt{DaTaReach}$ and $\texttt{DaTaControl}$, to over-approximate the reachable set and design control signals for the system on the fly. $\texttt{DaTaReach}$ constructs a differential inclusion that contains the unknown dynamics. Then, in a discrete-time setting, it over-approximates the reachable set through interval Taylor-based methods applied to systems with dynamics described as differential inclusions. We provide a bound on the time step size that ensures the correctness and termination of $\texttt{DaTaReach}$. $\texttt{DaTaControl}$ enables convex-optimization-based control using the computed over-approximation and the receding-horizon control framework. Besides, $\texttt{DaTaControl}$ achieves near-optimal control and is suitable for real-time control of such systems. We establish a bound on its suboptimality and the number of primitive operations it requires to compute control values. Then, we theoretically show that $\texttt{DaTaControl}$ achieves tighter suboptimality bounds with an increasing amount of data and richer side information. Finally, experiments on a unicycle, quadrotor, and aircraft systems demonstrate the efficacy of both algorithms over existing approaches.

==> save_proofs.tex <==
\begin{proof}
    Given the knowledge that $f(x_i) \in \mathcal{F}_i$ and $G(x_i) \in \mathcal{G}_i$, we want to obtain intervals $C_{\mathcal{F}_i} \subseteq \mathcal{F}_i$ and $C_{\mathcal{G}_i} \subseteq \mathcal{G}_i$ that prune out non-admissible values of $f(x_i)$ and $G(x_i)$ using the knowledge that $\dot{x}_i = f(x_i) + G(x_i) u_i$. We first have that
    \begin{align*}
        f(x_i) = \dot{x}_i - G(x_i) u_i \in (\dot{x}_i - \mathcal{G}_i u_i) \cap \mathcal{F}_i = C_{\mathcal{F}_i}.
    \end{align*}
    Therefore, a similar reasoning using the tighter interval $C_{\mathcal{F}_i}$ provides that $G(x_i) u_i \in (\dot{x}_i - C_{\mathcal{F}_i}) \cap (\mathcal{G}_i u_i) = s_0$. It is important to note that plugging back $s_0$ instead of $\mathcal{G}_i u_i$ in the expression of $C_{\mathcal{F}_i}$ will not yield an interval tighter than $C_{\mathcal{F}_i}$. Therefore, $C_{\mathcal{F}_i}$ and $s_0$ are optimal. Next, we focus on the term $G(x_i) u_i \in s_0$. We have that
    \begin{align*}
        (G(x_i))_{k,1} (u_i)_1 &= (G(x_i) u_i)_k - \sum_{l > 1 } (G(x_i))_{k,l} (u_i)_l \\
        &\in \underbrace{\big( (s_0)_k - \sum_{l>1} (\mathcal{G}_i)_{k,l} u_l \big) \cap \big( (\mathcal{G}_i)_{k,1} u_1\big)}_{(C_{\mathcal{G}_i})_{k,1} u_1},
    \end{align*}
    and we can deduce that 
    \begin{align*}
        \sum_{l > 1 } (G(x_i))_{k,l} (u_i)_l &\in \underbrace{\big( (s_0)_k - (C_{\mathcal{G}_i})_{k,1} u_1 \big) \cap \big( \sum_{l>1} (\mathcal{G}_i)_{k,l} u_l \big)}_{(s_1)_k},
    \end{align*}
    for all $k \in \mathbb{N}_{[1,n]}$. Using the same argument as for the optimality of $s_0$ and $C_{\mathcal{F}_i}$, we can say that $s_1$ and $(C_{\mathcal{G}_i})_{k,1} u_1$ are optimal. Finally, we apply the previous step in a sequential manner for $p=2,\hdots,m$ to the equality $(G(x_i))_{k,p} (u_i)_p = \sum_{l > p-1 } (G(x_i))_{k,l} (u_i)_l - \sum_{l > p } (G(x_i))_{k,l} (u_i)_l$ in order to obtain optimal intervals $s_p$ and $(C_{\mathcal{G}_i})_{k,p} u_p$. The procedure described here is similar to the \texttt{HC4-Revise} algorithm~\cite{benhamou-contractor1999} where optimality was proven when each variable, in our case $f(x_i)$ and $G(x_i)$, appears only once in the definition of the constraint, in our case $\dot{x}_i = f(x_i) + G(x_i) u_i$. 
\end{proof}

\begin{proof}
    This is a direct result from combining the arithmetic of intervals and the definition of the Lipschitz bounds for each $f_k$ and $G_{k,l}$. Specifically, from the upper bound $L_{f_k}$ on the Lipschitz constant of $f_k$, we have that 
    \begin{align*}
        |(f(x))_k - (f(y))_k| \leq L_{f_k} \|x-y\|_2, \: \: \forall x,y \in \mathcal{X}.
    \end{align*}
    Hence, given a data $(x_i, C_{\mathcal{F}_i}, C_{\mathcal{G}_i}) \in \mathscr{E}_N$ and $x \in  \mathcal{X}$, we can write that $(f(x))_k \in (f(x_i))_k + L_{f_k} \|x-x_i\|_2 [-1,1]$, and therefore $(f(x))_k \in (C_{\mathcal{F}_i})_k + L_{f_k} \|x-x_i\|_2 [-1,1]$ since $f(x_i) \in C_{\mathcal{F}_i}$. The previous belonging relation is valid for every data $(x_i, C_{\mathcal{F}_i}, C_{\mathcal{G}_i)} \in \mathscr{E}_N$ and as a result $(f(x))_k \in (\boldsymbol{f}(x))_k$. The same reasoning applied to $L_{G_{k,l}}$ enables to show that $(G(x))_{k,l} \in (\boldsymbol{G}(x))_{k,l}$.
\end{proof}

\begin{proof}
    This result is a direct consequence of Lemma~\ref{lem:contraction} and Lemma~\ref{lem:overapprox-f-G}. First, we show that for all $(x_i, C_{\mathcal{F}_i}, C_{\mathcal{G}_i}) \in \mathscr{E}_N$ given by Algorithm~\ref{algo:overapprox-datapoints}, we have $f(x_i) \in C_{\mathcal{F}_i}$ and $G(x_i) \in C_{\mathcal{G}_i}$. Specifically, as a consequence of line~\ref{alg:update-ei} of Algorithm~\ref{algo:overapprox-datapoints} and Lemma~\ref{lem:overapprox-f-G}, we have that $f(x_i) \in \mathcal{F}_i$ and $G(x_i) \in \mathcal{G}_i$. Hence, by line~\ref{alg:contraction-f-G} and Lemma~\ref{lem:contraction}, we immediately have that $f(x_i) \in C_{\mathcal{F}_i}$ and $G(x_i) \in C_{\mathcal{G}_i}$. As a consequence of lines~\ref{alg:begin-init-e}--\ref{alg:end-init-e}, $\mathscr{E}_N$ can be used in Lemma~\ref{lem:overapprox-f-G} to conclude that $f(x) \in \boldsymbol{f}(x)$ and $G(x) \in \boldsymbol{G}(x)$ for all $x \in \mathcal{X}$. Therefore, using interval arithmetic, we have $\dot{x} = f(x) + G(x) u \in \boldsymbol{f}(x) + \boldsymbol{G}(x) u$. The lines~\ref{alg:while-begin}--\ref{alg:while-end} enable to obtain tighter sets $C_{\mathcal{F}_i}$ and $C_{\mathcal{G}_i}$ by combining the Lipschitz continuity, the trajectory, and the values $C_{\mathcal{F}_i}$ and $C_{\mathcal{G}_i}$ obtained during previous iterations. Hence, $\mathscr{E}_N$ is optimal given the the trajectory and the Lipschitz continuity since we have the optimality of $C_{\mathcal{F}_i}$ and $C_{\mathcal{G}_i}$ by Lemma~\ref{lem:contraction}.
\end{proof}

\begin{proof}
This is a direct application of the definition of the Lipschitz bounds of $f_k$ and $G_{k,l}$. Specifically, we have that
\begin{align}
    &|{(h(x_1,u_1))}_k - {(h(x_2,u_1))}_k| \nonumber\\ 
    &= |{(f(x_1) - f(x_2))}_k+ \sum_{l=1}^m  {((G(x_1) - G(x_2))}_{k,l} {(u_1)}_l | \nonumber\\
    &\leq |{(f(x_1) - f(x_2))}_k| + \sum_{l=1}^m | {((G(x_1) - G(x_2))}_{k,l}| |{(u_1)}_l| \nonumber\\
    &\leq \big(L_{f_k} + \sum_{l=1}^m L_{G_{k,l}} |{(u_1)}_l| \big) \|x_1-x_2\|_2, \label{eq:bounds-hi}
\end{align}
for all $k \in \mathbb{N}_{[1,n]}$. The last inequality is obtained by the definitions of $L_{f_k}$ and $L_{G_{k,l}}$. Hence, the inequality~\eqref{eq:maximum-variation-h} is immediate by the definition of $\|\cdot\|_2$ and the inequality~\eqref{eq:bounds-hi}.
\end{proof}

\begin{proof}
For all $t \in [t_i, t_i + \Delta t]$, we have that
\begin{align}
    &\|x(t) - x(t_i)\|_2 \nonumber \\
    &= \|\int_{t_i}^{t} h(x(s), u(s)) ds \|_2 \label{eq:pvarsol-solution-characteristic} \\
    &\leq \begin{aligned}[t]
            &\int_{t_i}^{t} \|h(x(s),u(s))-h(x(t_i),u(s))\|_2 ds \\
            &\quad +  \int_{t_i}^{t} \|h(x(t_i),u(s))\|_2 ds
           \end{aligned} \label{eq:pvarsol-triangle-inequality}\\
    &\leq \begin{aligned}[t]
                &\int_{t_i}^{t} \beta(u(s)) \|x(s)-x(t_i)\|_2 ds + \int_{t_i}^{t} \|h(x(t_i),u(s))\|_2 ds
            \end{aligned} \label{eq:pvarsol-lipschitz-bounds} \\
    &\leq \|\alpha_i\|_2 (t-t_i) + \int_{t_i}^t \beta_i \|x(s)-x(t_i)\|_2 ds. \label{eq:pvarsol-pre-gronwall} 
\end{align}
We obtain~\eqref{eq:pvarsol-solution-characteristic} since $x$ is a solution of~\eqref{eq:control-linearization}. The passage from~\eqref{eq:pvarsol-solution-characteristic} to~\eqref{eq:pvarsol-triangle-inequality} results from applying the triangle inequality. We use Lemma~\ref{lem:h-variation} with $x_1 = x(s)$, $x_2=x(t_i)$, and $u_1 = u(s)$ to obtain~\eqref{eq:pvarsol-lipschitz-bounds}. We obtain~\eqref{eq:pvarsol-pre-gronwall} by showing that the inequalities $\beta(u(s)) \leq \beta_i$ and $\|h(x(t_i),u(s))\|_2 \leq \|\alpha_i\|_2$ hold for all $s\in[t_i,t_i+\Delta t]$. Specifically, the former inequality trivially holds by upper-bounding $|{(u(s))}_l|$ in the expression of $\beta(u(s))$ with $|(\boldsymbol{v}([t_i,t_i+\Delta t]))_l| \geq \sup_{s\in [t_i,t_i+\Delta t]} |{(u(s))}_l|$. The latter inequality holds since
\begin{align*}
    &|{(h(x(t_i),u(s)))}_k| \\
    &= |{(f(x(t_i)))}_k + \sum_{l=1}^m {(G(x(t_i))}_{k,l} {(u(s))}_l| \\
    &\leq | \ \underbrace{{(f(x(t_i)))}_k + \sum_{l=1}^m |{(G(x(t_i))}_{k,l}| \sup_{s \in [t_i,t_i+\Delta t]} |{(u(s))}_l|}_{ \leq (\alpha_i)_k} \ |.
\end{align*}

The inequality~\eqref{eq:pvarsol-pre-gronwall} satisfies the condition~\eqref{eq:gronwall-inequality} of Lemma~\ref{lem:gronwall-lemma} with $\Psi (t) = \|x(t) - x(t_i)\|_2$, $\alpha (t) = \|\alpha_i\|_2 (t-t_i)$, and $\gamma(t) = \beta_i$. Thus, we have that
\begin{align}
    \|x(t) - x(t_i)\| \leq \begin{aligned}[t]
                            &\|\alpha_i\|_2 (t-t_i) \\
                            &+ \beta_i \|\alpha_i\|_2 \int_{t_i}^t (s-t_i) \mathrm{e}^{\beta_i(t-s)} ds.
                     \end{aligned} \label{eq:pvarsol-post-gronwall}
\end{align}
By integration by parts, we have that
\begin{align}
    \int_{t_i}^t (s-t_i) \mathrm{e}^{\beta_i(t-s)} ds &= - \frac{t-t_i}{\beta_i} + \frac{1}{\beta_i}\int_{t_i}^t \mathrm{e}^{\beta_i(t-s)} ds \nonumber\\
     &= -\frac{t-t_i}{\beta_i} + \frac{\mathrm{e}^{\beta_i (t-t_i)} - 1}{\beta_i^2}. \label{eq:pvarsol-integration-part}
\end{align}
Finally, by combining~\eqref{eq:pvarsol-integration-part} and~\eqref{eq:pvarsol-post-gronwall}, we obtain~\eqref{eq:max-variation-solution}.
\end{proof}

\begin{proof}
    The expression~\eqref{eq:explict-fixpoint} is derived by scaling adequately the bound~\eqref{eq:max-variation-solution} from Lemma~\ref{lem:rate-change-solution}. Specifically, we seek for an a priori rough enclosure $\mathcal{S}_i$ such that 
    \begin{equation}\label{eq:fixpoint-to-find}
        \mathcal{S}_i = \mathcal{R}_i^+ + \mu \frac{\overline{\alpha}_i}{\beta_i} (\mathrm{e}^{\beta_i \Delta t} - 1) [-1,1]^n,
    \end{equation}
    where $\mu > 0$ is a parameter to find in order for $\mathcal{S}_i$ to satisfy the fixed-point equation~\eqref{eq:apriori-enclosure-control-affine} and $\overline{\alpha}_i$ is given by 
    $$\overline{\alpha}_i = \sup_{x(t_i) \in \mathcal{R}_i^+} \| \ f(x(t_i)) + |G(x(t_i))|  \ |\boldsymbol{v}([t_i,t_i+\Delta t])| \ \|_2.$$
    We over-approximate the set $\mathscr{R}(h, \mathcal{S}_i \times \boldsymbol{v}([t_i,t_i+\Delta t]))$ as a function of $\Delta t$, $\beta_{t_i,t_i+\Delta t}$, and $\boldsymbol{h} = \boldsymbol{f} + \boldsymbol{G} u$. For all $x_i \in \mathcal{R}_i^+$, $u_i \in \boldsymbol{v}([t_i,t_i+ \Delta t])$, and $s_i \in \mathcal{S}_i$, we have that
    \begin{align}
        \|h(s_i,u_i) - h(x_i,u_i)\|&\leq \beta_i \|s_i - x_i\| \label{eq:pfixpoint-var-h}\\
        &\leq  \sqrt{n} \mu \overline{\alpha}_i (\mathrm{e}^{\beta_i \Delta t} - 1). \label{eq:pfixpoint-bound-h}
    \end{align}
    The inequality~\eqref{eq:pfixpoint-var-h} comes from Lemma~\ref{lem:h-variation} with $\beta(u_i)$ upper-bounded by $\beta_i$ and the definition of $\mathcal{S}_i$~\eqref{eq:fixpoint-to-find} provides an upper bound on $\|s_i - x_i\|$ that yields~\eqref{eq:pfixpoint-bound-h}. Additionally, the inequality~\eqref{eq:pfixpoint-bound-h} implies that
    \begin{equation}
    \begin{aligned}[t]
         &\mathscr{R}(h, \mathcal{S}_i \times \boldsymbol{v}([t_i,t_i+\Delta t]))\\
         &\subseteq \boldsymbol{h}(\mathcal{R}_i^+,\boldsymbol{v}([t_i,t_i+\Delta t])) + \sqrt{n} \mu \overline{\alpha}_i (\mathrm{e}^{\beta_i \Delta t} - 1) [-1,1]^n.
    \end{aligned} \label{eq:pfixpoint-range-encllosure}
    \end{equation}
    Therefore, the set $\mathcal{S}_i$ given by~\eqref{eq:fixpoint-to-find} satisfies the fixed-point equation~\eqref{eq:apriori-enclosure-control-affine} if
    \begin{equation}
        \begin{aligned}[t]
            & [0, \Delta t] \Big(  \boldsymbol{h}(\mathcal{R}_i^+,\boldsymbol{v}([t_i,t_i+\Delta t])) + \sqrt{n} \mu \overline{\alpha}_i (\mathrm{e}^{\beta_i \Delta t} - 1) [-1,1]^n \Big) \\
            & \subseteq \mu \frac{\overline{\alpha}_i}{\beta_i} (\mathrm{e}^{\beta_i \Delta t} - 1) [-1,1]^n. 
        \end{aligned}\label{eq:pfixpoint-rincl}
    \end{equation}
    For notation brevity, let $c_1 = \overline{\alpha}_i (\mathrm{e}^{\beta_i \Delta t} - 1)$. Observe that $[0,\Delta t][\underline{\mathcal{A}},\overline{\mathcal{A}}] = [\min (0,\underline{\mathcal{A}}), \max (0,\overline{\mathcal{A}})]$. We use the observation to find $\mu >0$ such that the inclusion~\eqref{eq:pfixpoint-rincl} holds. That is, the inequalities 
    \begin{align*}
        &\Delta t \Big( \overline{{(\boldsymbol{h}(\mathcal{R}_i^+,\boldsymbol{v}([t_i,t_i+\Delta t])))}_k} + \sqrt{n} \mu c_1 \Big) \leq \frac{\mu c_1}{\beta_i} \\
        &\Longleftrightarrow (\frac{1}{\Delta t \beta_i} - \sqrt{n}) \mu \geq \frac{1}{c_1} \overline{{(\boldsymbol{h}(\mathcal{R}_i^+,\boldsymbol{v}([t_i,t_i+\Delta t])))}_k}
    \end{align*}
    and 
    \begin{align*}
        &\Delta t \Big( \underline{{(\boldsymbol{h}(\mathcal{R}_i^+,\boldsymbol{v}([t_i,t_i+\Delta t])))}_k} - \sqrt{n} \mu c_1 \Big) \geq -\frac{\mu c_1}{\beta_i} \\
        &\Longleftrightarrow (\sqrt{n} - \frac{1}{\Delta t \beta_i}) \mu \geq \frac{1}{c_1} \underline{{(\boldsymbol{h}(\mathcal{R}_i^+,\boldsymbol{v}([t_i,t_i+\Delta t])))}_k}
    \end{align*}
    hold for all $k \in \mathbb{N}_{[1,n]}$. Therefore, for a step size $\Delta t$ satisfying~\eqref{eq:step-size-bound}, $\mu$ given by 
    \begin{align*}
        \mu = \frac{\|\boldsymbol{f}(\mathcal{R}_i^+) + \boldsymbol{G}(\mathcal{R}_i^+) \boldsymbol{v}([t_i,t_i+\Delta t])\|_{\infty}}{c_1 (\frac{1}{\Delta t \beta_i} - \sqrt{n})}
    \end{align*}
    satisfies the above inequalities. Thus, the inclusion~\eqref{eq:pfixpoint-rincl} holds and the set $\mathcal{S}_i$ is solution of the fixed-point equation~\eqref{eq:apriori-enclosure-control-affine}. By replacing $\mu$ in $\mathcal{S}_i$ given by~\eqref{eq:fixpoint-to-find}, we obtain the expression~\eqref{eq:explict-fixpoint}.
\end{proof}

\begin{proof}
    This proof applies the interval Taylor-based method of Section~\ref{sec:prelem-taylor-method} on the dynamics described by $\dot{x}\in \boldsymbol{f}(x) + \boldsymbol{G}(x) u$. Clearly, $\boldsymbol{h}(\mathcal{Z},\mathcal{W}) = \boldsymbol{f}(\mathcal{Z}) + \boldsymbol{G}(\mathcal{Z}) \mathcal{W}$ is an interval extension of $h(x,u) = f(x) + G(x) u$.
    Hence, the set $\mathcal{S}_i$ solution of~\eqref{eq:fix-point-rough} or given by~\eqref{eq:explict-fixpoint} is an a priori rough enclosure as it satisfies the fixed-point equation~\eqref{eq:rough-enclosure}. We use a Taylor expansion~\eqref{eq:taylor-expansion} of order $D=2$ to obtain
    \begin{align}
        \mathcal{R}^+_{i+1} &\subseteq  \mathcal{R}^+_i + \Delta t \Big( \boldsymbol{h}(\mathcal{R}^+_i,\boldsymbol{v}(t_i)) \Big) + \frac{\Delta t^2}{2} \Big(  \boldsymbol{\frac{\partial h }{\partial x}}  \boldsymbol{h}  \Big) (\mathcal{S}_i, \mathcal{V}_i)
                                              \nonumber \\
                                              & \quad \quad \quad + \frac{\Delta t^2}{2} \Big( \boldsymbol{\frac{\partial h }{\partial u}} \Big) (\mathcal{S}_i, \mathcal{V}_i) \mathcal{V}_i^{(1)}, \label{eq:taylor-2-order}
    \end{align}
    where $\boldsymbol{\frac{\partial h }{\partial x}}$ and $\boldsymbol{\frac{\partial h }{\partial u}}$ are interval extensions of $\frac{\partial h }{\partial x}$ and $\frac{\partial h }{\partial u}$, respectively. We have that $\boldsymbol{G}$ is an interval extension of $\frac{\partial h }{\partial u}$ as
    \begin{align} \label{eq:proof-partial-der-u-extension}
        \frac{\partial h }{\partial u} (x,u) = G(x) \in \boldsymbol{G}(x) \Longrightarrow \boldsymbol{\frac{\partial h }{\partial u}}  = \boldsymbol{G}. 
    \end{align}
    Furthermore, for all $k,p \in \mathbb{N}_{[1,n]}$, $x \in \mathcal{X}$ and $u \in  \mathcal{U}$, we have 
    \begin{align*}
        \frac{\partial h_k}{\partial x_p}(x,u) = \frac{\partial f_k}{\partial x_p}(x,u) + \sum_{l=1}^m \frac{\partial G_{k,l}}{ \partial x_p}(x,u) u_l.
    \end{align*}
    Thus, a consequence of \textit{Rademacher's theorem}~\cite[Theorem $3.1.6$]{Federer:228981} enables to write that
    \begin{align*}
        \frac{\partial f_k}{\partial x_p}  \in  L_{f_k} [-1, 1] \text{ and }
        \frac{\partial G_{k,l}}{ \partial x_p}  \in L_{G_{k,l}}[-1,1].
    \end{align*}
    Therefore, we have that $\boldsymbol{\frac{\partial h }{\partial x}}(\mathcal{S}_i, \mathcal{V}_i) = \mathcal{J}_f + \mathcal{J}_G \mathcal{V}_i$.
    % \begin{equation} \label{eq:proof-partial-der-x-extension}
    %     \boldsymbol{\frac{\partial h }{\partial x}} (\mathcal{S}_i, \mathcal{V}) = \mathcal{J}_f +  \mathcal{J}_G \mathcal{V}.
    % \end{equation}
    Finally, merging $\boldsymbol{\frac{\partial h }{\partial x}}$ and $\boldsymbol{\frac{\partial h }{\partial u}}$ into~\eqref{eq:taylor-2-order} provides the over-approximating set~\eqref{eq:over-approx-next-state}. 
\end{proof}

\begin{proof}
    We  apply Theorem~\ref{thm:over-approximation-state} with $\mathbb{V} = \{u_i\}$. Specifically, since $u$ is such that  $\dot{u}(t) = 0$ for all $t \in [t_i , t_{i}+\Delta t]$,  we have that $\boldsymbol{v}(t_i)=u_i$, $\boldsymbol{v}([t_i,t_i+\Delta t]) = u_i$, and $\boldsymbol{v}^{(1)}([t_i,t_i+\Delta t]) = 0$. Applying Theorem~\ref{thm:over-approximation-state}, $\mathcal{R}^+_{i+1}$ as a function of $u_i$ is therefore reduced to a term independent of $u_i$, a term linear in $u_i$, and a term quadratic in $u_i$.
    
    Specifically, it is immediate from~\eqref{eq:over-approx-next-state} that the term independent of $u_i$ is given by $\mathcal{B}_i$~\eqref{eq:linear-over-const}. The term linear in $u_i$ is
    \begin{align}
        & \big( \boldsymbol{G} (\mathcal{R}^+_i) \Delta t \big) u_i  +  \big( \mathcal{J}_G u_i \boldsymbol{f} (\mathcal{S}_j) + \mathcal{J}_f \boldsymbol{G}(\mathcal{S}_j) u_i \big) \frac{\Delta t^2}{2}. \label{eq:full-linear-term}
    \end{align}
    The $k$-th component of $\mathcal{J}_G u_i \boldsymbol{f} (\mathcal{S}_i)$ is given by
    \begin{align}
        \sum_{p=1}^n {(\mathcal{J}_G u_i)}_{k,p} (\boldsymbol{f} {(\mathcal{S}_i))}_p &= \sum_{p=1}^n \big( \sum_{l=1}^m {(\mathcal{J}_G)}_{k,l,p} {(u_i)}_l \big) (\boldsymbol{f} {(\mathcal{S}_i))}_p \nonumber \\
        &= \sum_{l=1}^m \big( \underbrace{\sum_{p=1}^n  {(\mathcal{J}_G)}_{k,l,p} {(\boldsymbol{f} (\mathcal{S}_i))}_p}_{{(\mathcal{J}_G^\textrm{T} \boldsymbol{f}(\mathcal{S}_i))}_{k,l}} \big) {(u_i)}_l \nonumber \\
        &= {(\mathcal{J}_G^\textrm{T} \boldsymbol{f}(\mathcal{S}_i) u_i)}_k. \label{eq:linear-reordering}
    \end{align}
    The quadratic term $0.5 \Delta t^2 \mathcal{J}_G u_i \boldsymbol{G} (\mathcal{S}_i) u_i$ in $u_i$ satisfies
    \begin{align}
         \mathcal{J}_G u_i \boldsymbol{G} (\mathcal{S}_i) u_i &\subseteq  \mathcal{J}_G \mathcal{U} \boldsymbol{G}(\mathcal{S}_i) u_i, \label{eq:a1-formula}\\
         \mathcal{J}_G u_i \boldsymbol{G} (\mathcal{S}_i) u_i &\subseteq  \mathcal{J}_G u_i \boldsymbol{G}(\mathcal{S}_i) \mathcal{U} =  \mathcal{J}^{\textrm{T}}_G \boldsymbol{G}(\mathcal{S}_i) \mathcal{U} u_i. \label{a2-formula}
    \end{align}
    Henceforth, by combining~\eqref{eq:full-linear-term},~\eqref{eq:linear-reordering}, and~\eqref{eq:a1-formula}, the linear and quadratic terms in $u_i$ of $\mathcal{R}^+_{i+1}$ can be over-approximated by the linear term  $\mathcal{A}^+_i u_i$ with $\mathcal{A}^+_i$ given by~\eqref{eq:linear-over-lin-term-1}. Similar story, using~\eqref{a2-formula}, holds for proving that the linear and quadratic terms in $u_i$ can be also over-approximated by $\mathcal{A}^-_i u_i$ with $\mathcal{A}^-_i$ given by~\eqref{eq:linear-over-lin-term-2}. Hence, we deduce the intersection in~\eqref{eq:linear-over-approx}. 
\end{proof}

\begin{proof}
    For any $x^+_{i+1} = b_i + A^+_i u_i  \in \mathcal{B}_i + \mathcal{A}^+_i u_i$ and $\hat{x}^+_{i+1} = \hat{b}_i + \hat{A}_i^+ u_i \in \mathcal{B}_i + \mathcal{A}^+_i u_i$ with $u_i \in \mathcal{U}$, we have that 
    \begin{align}
        & \quad |c(\cdot, u_i , x^+_{i+1}) - c(\cdot,u_i,\hat{x}^+_{i+1})| \nonumber \\
        &= \big| \begin{bmatrix} x^+_{i+1} \\ u_i \end{bmatrix}^{\mathrm{T}} \begin{bmatrix} Q & S \\ S^{\mathrm{T}}  & R\end{bmatrix} \begin{bmatrix} x^+_{i+1} \\ u_i \end{bmatrix} 
        - \begin{bmatrix} \hat{x}^+_{i+1} \\ u_i \end{bmatrix}^{\mathrm{T}} \begin{bmatrix} Q & S \\ S^{\mathrm{T}}  & R\end{bmatrix} \begin{bmatrix} \hat{x}^+_{i+1} \\ u_i \end{bmatrix} \nonumber \\
        & \quad \quad  + \begin{bmatrix} q \\ r\end{bmatrix}^{\mathrm{T}} \begin{bmatrix}  x^+_{i+1} - \hat{x}^+_{i+1} \\ 0 \end{bmatrix} \big| \nonumber \\
        &=  \big| \big( x^+_{i+1} - \hat{x}^+_{i+1} \big)^{\mathrm{T}}  \big( Q \big( x^+_{i+1} + \hat{x}^+_{i+1} \big) +  2 S u_i + q \big) \big| \nonumber \\
        &\leq \big(\| (b_i - \hat{b}_i) + (A^+_i - \hat{A}^+_i) u_i \|_2 \big) \nonumber \\ 
        &\quad \quad \big( \|  Q \big( (b_i + \hat{b}_i) + (A^+_i + \hat{A}^+_i) u_i \big) + 2 S u_i + q \|_2 \big) \label{eq:diff-cost}.
    \end{align}
    By definition of the width  $w$, $|b_i - \hat{b}_i| \leq w(\mathcal{B}_i)$ and $|A^+_i - \hat{A}^+_i| \leq w(\mathcal{A}^+_i)$. Hence, we can deduce that
    \begin{align}
        \| (b_i - \hat{b}_i) + (A^+_i - \hat{A}^+_i) u_i \|_2 \leq \| w(\mathcal{B}_i) + w(\mathcal{A}^+_i)|\mathcal{U}| \|_2. \label{eq:first-term}
    \end{align}
    Furthermore, interval arithmetic provides that
    \begin{align*}
        (b_i + \hat{b}_i) + (A^+_i + \hat{A}^+_i) u_i \in \big( 2\mathcal{B}_i + 2\mathcal{A}^+_i u_i \big)  \cap  2\mathcal{X}.
    \end{align*}
    Hence, we have
    \begin{align}
        &\begin{aligned}[t] \|& 2 S u_i + q + Q \big( (b_i + \hat{b}_i) + (A^+_i + \hat{A}^+_i) u_i \big) \|_2  \\
        &\quad \leq \| 2 |S \mathcal{U}| + q +  2 | Q (\mathcal{B}_i + \mathcal{A}^+_i \mathcal{U} )| \|_2, 
        \end{aligned} \label{eq:second-term-unbound} \\
        &\begin{aligned}[t]
        &\| 2 S u_i + q + Q \big( (b_i + \hat{b}_i) + (A^+_i + \hat{A}^+_i) u_i \big) \|_2 \\
        &\quad \leq  \| 2|S \mathcal{U}| + q +  2| Q \mathcal{X}|\|_2. \label{eq:second-term-bound}
        \end{aligned}
    \end{align}
    Therefore, combining~\eqref{eq:second-term-bound} and~\eqref{eq:second-term-unbound}, we have that
    \begin{align}
        &\| 2 S u_i + q + Q \big( (b_i + \hat{b}_i) + (A^+_i + \hat{A}^+_i) u_i \big) \|_2 \leq M^+_i. \label{eq:m_plus_bound}
    \end{align}
    As a consequence of~\eqref{eq:diff-cost},~\eqref{eq:first-term}, and~\eqref{eq:m_plus_bound}, we can write 
    \begin{align}
        |c(\cdot, u_i , x^+_{i+1}) - c(\cdot,u_i,\hat{x}^+_{i+1})| \leq \| w(\mathcal{B}_i) + w(\mathcal{A}^+_i)|\mathcal{U}| \|_2 M_i^+. \label{eq:bound-diff-cost}
    \end{align}
    
    Let $u^*_i$ be the optimal solution of the one-step optimal control problem~\eqref{eq:one-step-optimal-control} and $x_{i+1}(u^*_i) \in \mathcal{B}_i + \mathcal{A}^+_i u^*_i$ be the corresponding unknown next state. By optimality of $u^*_i$, we have that $c(x_i, u^*_i, x_{i+1}(u^*_i)) \leq c(x_i, u_i, x_{i+1}(u_i))$ for all $u_i \in \mathcal{U}$. If $\hat{u}_i$ is the optimal solution of the optimistic control problem~\eqref{eq:optimistic-control-problem} and $\hat{x}_{i+1}(\hat{u}_i) \in \mathcal{B}_i + \mathcal{A}^+_i u^*_i$ is the known next state for which the optimum of~\eqref{eq:optimistic-control-problem} is attained, then
    \begin{align*}
       |c_i^{\star} - c_i^{\mathrm{opt}}| &=  | c(x_i, u^*_i, x_{i+1}(u^*_i)) - c(x_i, \hat{u}_i, \hat{x}_{i+1}(\hat{u}_i)) |\\
                            &\leq  | c(x_i, \hat{u}_i, x_{i+1}(\hat{u}_i)) - c(x_i, \hat{u}_i, \hat{x}_{i+1}(\hat{u}_i)) | \\
                            &\leq \| w(\mathcal{B}_i) + w(\mathcal{A}^+_i)|\mathcal{U}| \|_2 M^+_i.
    \end{align*}
    Similarly, using $\mathcal{A}^-_i$ instead of $\mathcal{A}^+_i$, we can prove that $|c_i^{\star} - c_i^{\mathrm{opt}}| \leq \| w(\mathcal{B}_i) + w(\mathcal{A}^-_i)|\mathcal{U}| \|_2 M^-_i$. Hence we obtain the suboptimality bounds~\eqref{eq:bounds-approximate} for the optimistic control problem.
    
    Finally, let $\hat{u}_i$ be the optimal solution of the idealistic control problem~\eqref{eq:idealistic-control-problem} and $\hat{x}_{i+1}(\hat{u}_i) = b^{\mathrm{ide}}_i + A^{\mathrm{ide}}_i \hat{u}_i$ be the next state for which the optimum is attained. We have that
    \begin{align*}
        |c_i^{\mathrm{ide}} - c_i^{\star}| &= \begin{cases} c_i^{\mathrm{ide}} - c(x_i, u^{\star}_i, x_{i+1}(u^*_i)),& \text{if } c_i^{\mathrm{ide}} \geq c_i^{\star} \\ c_i^{\star} - c(x_i, \hat{u}_i,\hat{x}_{i+1}(\hat{u}_i) ),& \text{otherwise} \end{cases} \\
        &\leq \begin{cases} c(x_i, u^{\star}_i, \hat{x}_{i+1}(u^{\star}_i)) - c(x_i, u^{\star}_i, x_{i+1}(u^*_i)),\\ \quad \text{if } c_i^{\mathrm{ide}} \geq c_i^{\star} \\ c(x_i, \hat{u}_i, x_{i+1}(\hat{u}_i))  - c(x_i, \hat{u}_i,\hat{x}_{i+1}(\hat{u}_i) ), \\ \quad \text{otherwise} \end{cases} \\
        &\leq \| w(\mathcal{B}_t) + w(\mathcal{A}_t)|\mathcal{U}| \|_2 M_t,
    \end{align*}
    where the second inequality follows from the definition of optimality of~\eqref{eq:one-step-optimal-control} and~\eqref{eq:idealistic-control-problem}, and the last inequality follows similarly to the inequalities obtained for the optimistic suboptimality bounds. 
\end{proof}

\begin{proof}
    We use the interval arithmetic to characterize exactly the belonging relations $x_{i+1} \in \mathcal{B}_i + \mathcal{A}^+_i u_i$ and $x_{i+1} \in \mathcal{B}_i + \mathcal{A}^-_i u_i$ in term of linear constraints. Specifically, since $(\mathcal{A}^+_i u_i)_k = \sum_{l=1}^m (\mathcal{A}^+_i)_{k,l} (u_i)_l$, interval arithmetic provides upper and lower bound on each term $(\mathcal{A}^+_i)_{k,l} (u_i)_l$ as follows
    \begin{equation*}
        \begin{cases}   
            (\mathcal{A}^+_i)_{k,l} (u_i)_l = [\underline{(\mathcal{A}^+_i)_{k,l}} (u_i)_l,\overline{(\mathcal{A}^+_i)_{k,l}} (u_t)_l], &\text{if }  (\mathcal{U})_l \geq 0 \\[3pt]
            
            (\mathcal{A}^+_i)_{k,l} (u_i)_l = [\overline{(\mathcal{A}^+_i)_{k,l}} (u_t)_l, \underline{(\mathcal{A}^+_i)_{k,l}} (u_i)_l], &\text{otherwise.} \end{cases}
    \end{equation*}
    We can deduce that $\overline{\mathcal{A}^+_i u_i} = A_i^{\mathrm{s}+} u_i$ and $\underline{\mathcal{A}^+_i u_i} = A_i^{\mathrm{l}+} u_i$. Similarly, it is easy to prove that $\overline{\mathcal{A}^-_i u_i} = A_i^{\mathrm{s}-} u_i$ and $\underline{\mathcal{A}^-_i u_i} = A_i^{\mathrm{l}-} u_i$. As a consequence, the optimistic control problem~\eqref{eq:optimistic-control-problem} can be immediately reformulated as the convex quadratic programming problem~\eqref{eq:optimistic-expr-qp}. 
    
    Additionally, we have that
    \begin{align*}
        &c(x_i, u_i, b_i^{\mathrm{ide}} + A_i^{\mathrm{ide}} u_i) \\
        &= (b_i^{\mathrm{ide}} + A_i^{\mathrm{ide}} u_i)^{\mathrm{T}} Q (b_i^{\mathrm{ide}} + A_i^{\mathrm{ide}} u_i) + u_i^{\mathrm{T}} R u_i \\
        &\quad \: + 2 (b_i^{\mathrm{ide}} + A_i^{\mathrm{ide}} u_i)^{\mathrm{T}} S u_i + (b_i^{\mathrm{ide}} + A_i^{\mathrm{ide}} u_i)^{\mathrm{T}} q + r^{\mathrm{T}} u_i \\
        &= u_i^{\mathrm{T}}\Big((A_i^{\mathrm{ide}})^{\mathrm{T}} Q A_i^{\mathrm{ide}} + 2 (A_i^{\mathrm{ide}})^{\mathrm{T}} S + R \Big) u_i \\
        &\quad \: + \Big(  2(b_i^{\mathrm{ide}})^{\mathrm{T}} \big( S + Q A_i^{\mathrm{ide}} \big) + q^{\mathrm{T}} A_i^{\mathrm{ide}} + r^{\mathrm{T}} \Big) u_i \\
        &\quad \: + (b_i^{\mathrm{ide}})^{\mathrm{T}} Q b_i^{\mathrm{ide}} + q^{\mathrm{T}} b_i^{\mathrm{ide}} \\
        &= u_i^{\mathrm{T}} Q_i u_i + q_i^{\mathrm{T}} u_i + p_i.
    \end{align*}
    Hence we obtain the cost function of the idealistic control problem~\eqref{eq:qp-midpoint}. Therefore, it remains to prove that the matrix $Q_i$ is positive semidefinite. Let prove that $u_i^{\mathrm{T}} Q_i u_i \geq 0$ for all $u_i \in \mathbb{R}^m$. Since we have that 
    $$ \begin{bmatrix} Q & S \\ S^{\mathrm{T}}  & R\end{bmatrix} \succeq 0, $$
    we can deduce that 
    $$ \begin{bmatrix} A_i^{\mathrm{ide}} u_i \\ u_i\end{bmatrix}^{\mathrm{T}} \begin{bmatrix} Q & S \\ S^{\mathrm{T}}  & R\end{bmatrix} \begin{bmatrix} A_i^{\mathrm{ide}} u_i \\ u_t\end{bmatrix} \geq 0, $$
    for all $u_i \in \mathbb{R}^m$. Expanding the expression above immediately provides that $u_i^{\mathrm{T}} Q_i u_i \geq 0$ for all $u_i \in \mathbb{R}^m$.
\end{proof}
